Learning Semantics, Not Addresses: Runtime Neural Prefetching for Far Memory

Memory prefetching has long boosted CPU caches and is increasingly vital for far-memory systems, where large portions of memory are offloaded to cheaper, remote tiers. While effective prefetching requires accurate prediction of future accesses, prior ML approaches have been limited to simulation or small-scale hardware. We introduce FarSight, the first Linux-based far-memory system to leverage deep learning by decoupling application semantics from runtime memory layout. This separation enables offline-trained models to predict access patterns over a compact ordinal vocabulary, which are resolved at runtime through lightweight mappings. Across four data-intensive workloads, FarSight delivers up to 3.6x higher performance than the state-of-the-art.

==> fig-futuremap-swap.tex <==
{
\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/futuremap-swap.pdf}}
\mycaption{fig-futuremap-swap}{Indirected and Swappable Future Maps.}
{
Application pages have one-to-one mapping to future-map roots based on their virtual page number (VPN), while the mapping from future-map roots to future maps is dynamic.
On the left, the blue page (VPN 3) and its associated futuremap are swapped out.
On the right, the yellow page (VPN k) and its futuremap is swapped in.
}
\end{center}
\end{figure}
}

==> fig-pattern-pr.tex <==
{
\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{Figures/patterns.pdf}}
\mycaption{fig-pattern}{Example Memory Access Sequence over Time}
{Captured by tracing page access sequence during execution.}
\end{center}
\end{figure}
}



==> fig-predictunit.tex <==
{
\begin{figure}[th]
\begin{center}
\centerline{\includegraphics[width=0.85\columnwidth]{Figures/predictunit.pdf}}
\mycaption{fig-predictunit}{\sys\ Prediction Unit}
{
Illustration of reduction from using all memory addresses to misses to missed chunks.
Each color represents a distinct chunk. Different shades of a color represents addresses within a chunk.
}
\end{center}
\end{figure}
}
%\notevikranth{I don’t get this diagram in isolation here. }

